Cycles in adversarial regularized learning

Regularized learning is a fundamental technique in online optimization, machine learning and many other fields of computer science. A natural question that arises in these settings is how regularized learning algorithms behave when faced against each other. We study a natural formulation of this problem by coupling regularized learning dynamics in zero-sum games. We show that the system's behavior is Poincar\'e recurrent, implying that almost every trajectory revisits any (arbitrarily small) neighborhood of its starting point infinitely often. This cycling behavior is robust to the agents' choice of regularization mechanism (each agent could be using a different regularizer), to positive-affine transformations of the agents' utilities, and it also persists in the case of networked competition, i.e., for zero-sum polymatrix games.

==> Boundary.tex <==
%----------------------------------------------------------------------
%%% BOUNDARY EQUILIBRIA
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


In this section, we will argue that in the case where there exist no Nash equilibrium in the interior of the state space (i.e. fully mixed strategy profile) then the dynamics converge to the boundary.

\begin{definition}
A strategy $\pure_\play$ of agent $\play \in \{1,2\}$ in a zero sum game is called {\bf essential} if there exists a Nash equilibrium strategy of agent $\play$ that plays it with positive probability.  A strategy that is not essential is called {\bf nonessential}.
\end{definition}

\begin{lemma}
\label{lem:Farka_eq}
Let $\game$ be a $2$-player zero-sum game (that does not admit an interior \acl{NE}),
then there exists a mixed Nash equilibrium $(\strat_{1}, \strat_{2})$ such that i) each agent plays each of his essential strategies with positive probability and ii) for each agent deviating to a non-essentially strategy results to a strictly worse performance than the value of the game.\end{lemma}

\begin{proof}
We assume without loss of generality that the value of the zero-sum game is zero. 
and that the first agent is a maximizing agent.
Let $A$ be the payoff matrix of the first agent and hence $A^{T}=A$ the payoff matrix of the second/minimizing agent. We will show first that for any nonessential strategy $\pure_\play$ of each agent there exists a Nash equilibrium strategy of his opponent such that the expected performance of $\pure_\play$ is strictly worse than the value of the game (i.e. zero).   

It suffices to argue this for the first agent. Let  $\pure_\play$ be one of his nonessential strategies then by definition there does not exist any Nash equilibrium strategy of that agent that chooses  $\pure_\play$ with positive probability. This is equivalent to the negation of the following statement:

There exists a $\mathbf{x} \in \mathbb{R}^{m}$ such that $\mathbf{P}^{\top}\mathbf{x} \geq 0$ and $\mathbf{b}^{\top}\mathbf{x}  < 0$


\noindent
where 

\begin{equation} \label{first_condition}
 \mathbf{P}^{\top} =\begin{pmatrix}                                            
                                                   \mathbf{A}^{\top} \\ 
                                                    \mathbf{I}_{m\times m}                                               
                                                    \end{pmatrix} = \begin{pmatrix}
                                  a_{11}& a_{21} & \ldots & a_{m1}\\
                                   \vdots & \vdots & \ldots & \vdots\\
                                  a_{1n}& a_{2n} & \ldots & a_{mn}\\
                                    1 & 0 & \ldots & 0 \\
                                  0&  1& \ldots &   0\\
                                  \vdots & \vdots & \ldots & \vdots\\
                                  0&  0& \ldots &   1\\ 
                                \end{pmatrix} ,
\end{equation}

\noindent
and
$\mathbf{b}= -\mathbf{e}_{i} = (0, \dots, 0, -1, 0, \dots, 0)^T$, the standard basis vector of dimension $m$ that ``chooses" the $\play$-th strategy.  By Farkas' lemma,  there exists a $\mathbf{y} \in \mathbb{R}^{m+n}$ such that $\mathbf{Py} = \mathbf{b}$ and $\mathbf{y} \geq 0$. It is convenient to express $\mathbf{y}= (\mathbf{z}; \mathbf{w})$ where    $\mathbf{z} \in  \mathbb{R}^{n}$ and $\mathbf{w} \in  \mathbb{R}^{m}$.
Hence, for all $j \neq \play \in \{1,2, \dots, m\}: \mathbf{(Py)}_j= \mathbf{(Az)}_j+\mathbf{w}_j=0$ and thus $\mathbf{(Az)}_j\leq 0$. Finally, for $j=\play: \mathbf{(Py)}_\play= \mathbf{(Az)}_\play+\mathbf{w}_\play=-1$ and thus $\mathbf{(Az)}_\play<0$. Hence $\mathbf{z}$ is a Nash equilibrium strategy for the second player such that when the first agent chooses the nonessential strategy $\pure_\play$ he receives payoff which is strictly worse than his value (zero).

To complete the proof, for each essential strategy of the first agent there exists one equilibrium strategy of his that chooses it with positive probability (by definition). Similarly, for each nonessential strategy of the second agent there exists one equilibrium strategy of the first agent such that makes the expected payoff of that nonessential strategy strictly worse than the value of the game. The barycenter of all the above equilibrium strategies is still an equilibrium strategy (by convexity) and has all the desired properties.
\end{proof}


We will now use the \eqref{eq:FRL-z} representation of the dynamics to show that in this case they converge to the boundary.
 %We now proceed to show that every solution orbit $z(t)$ of \eqref{eq:FRL-z} is precompact, i.e. $\sup_{t\geq0} \norm{z(t)} < \infty$.
To that end, we first show that the coupling function $\fench(y) = \sum_{\play\in\players} \bracks{h_{\play}^{\ast}(y_{\play}) - \braket{y_{\play}}{\eq_{\play}}}$ defined in \eqref{eq:Fenchel} given any fully mixed initial condition strictly increases under \eqref{eq:FRL} when $\game$ is a $2$-player zero-sum game that does not have an equilibrium of full support. 

By \ref{lem:Farka_eq} there exists a mixed Nash equilibrium $(\eq_{1}, \eq_{2})$ such that i) each agent plays each of his essential strategies with positive probability and ii) for each agent deviating to a non-essentially strategy results to a strictly worse performance than the value of the game. As a result, any agent playing an interior (fully mixed) strategy against such an equilibrium strategy must receive less utility than their value.
Thus, we have

\begin{flalign}
\label{eq:dFench2}
\frac{d\fench}{dt}
	= \braket{\dot y}{\nabla\fench(y)}
	&= \sum_{\play\in\players} \braket{\payv_{\play}(x)}{\nabla h_{\play}^{\ast}(y_{\play}) - \eq_{\play}}
	\notag\\
	&= \sum_{\play\in\players} \braket{\payv_{\play}(x)}{x_{\play} - \eq_{\play}}
	= \braket{\payv_{1}(x)}{x_{1} - \eq_{1}}
		+ \braket{\payv_{2}(x)}{x_{2} - \eq_{2}}
	\notag\\
	&= \pay_{1}(x_{1},x_{2}) - \pay_{1}(\eq_{1},x_{2})
		+ \pay_{2}(x_{1},x_{2}) - \pay_{2}(x_{1},\eq_{2})
	\notag\\
	&= - \pay_{1}(\eq_{1},x_{2})
		 - \pay_{2}(x_{1},\eq_{2})
	\notag\\
	&< - \pay_{1}(\eq_{1},\eq_{2})
		 - \pay_{2}(\eq_{1},\eq_{2})
	\notag\\
	&= 0,
\end{flalign}
where we used the fact that $\choice_{\play} = \nabla h_{\play}^{\ast}$ in the first line (cf. \cref{app:aux}), and the assumption that $\eq$ is a \acl{NE} of a $2$-player zero-sum game such that  any agent playing an interior (fully mixed) strategy against such an equilibrium strategy must receive less utility than their value (and hence the agent himself receives more utility than the value of the game).
We thus conclude that $\fench(y(t))$ strictly increases under \eqref{eq:FRL}, as claimed.





%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\GP{The following is the proof for the replicator alone. I.e. the argument that the replicator converges to the boundary.}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



Next we prove  the following technical lemma:
%, whose proof can be found in \cite{Akin84} but is also provided here for completeness:

\PM{New lemma below.}

\begin{lemma}
\label{lem:derivative}
Suppose that $\lyap\from[0,\infty)\to\R$ is differentiable with Lipschitz continuous derivative.
If $\lim_{t\to\infty} \lyap(t)$ exists and is finite, we have $\lim_{t\to\infty} \lyap'(t) = 0$.
\end{lemma}

\begin{proof}
Assume ad absurdum that $\lim_{t\to\infty} \lyap'(t) \neq 0$.
Then, without loss of generality, we may assume there exists some $\eps>0$ and an increasing sequence $t_{n}\uparrow\infty$ such that $\lyap'(t_{n}) \geq \eps$ for all $n\in\N$.
Thus, if $M$ denotes the Lipschitz constant of $\lyap'$ and $t\in[t_{n},t_{n} + \eps/(2M)]$, we readily obtain
\begin{equation}
\abs{\lyap'(t) - \lyap'(t_{n})}
	\leq M \abs{t - t_{n}}
	\leq M \cdot \frac{\eps}{2M}
	= \frac{\eps}{2}
\end{equation}
by the Lipschitz continuity of $\lyap'$.
Since $\lyap'(t_{n}) \geq \eps$ by assumption, we conclude that $\lyap'(t) \geq \eps/2$ for all $t\in[t_{n},t_{n}+\eps/(2M)]$.
Hence, by integrating, we get $\lyap(t_{n}+\eps/(2M)) \geq \lyap(t_{n}) + \eps/(2M) \cdot (\eps/2) = \lyap(t_{n}) + \eps^{2}/(4M)$ for all $n\in\N$.
Taking $n\to\infty$ and recalling that $\lyap_{\infty} \equiv \lim_{t\to\infty} \lyap(t)$ exists and is finite, we get $\lyap_{\infty} = \lyap_{\infty} + \eps^{2}/(4M) > \lyap_{\infty}$, a contradiction.
\end{proof}

%\begin{lemma}
%\label{eq:derivative}
%If $\lyap(t)$ is a twice differential function with uniformly bounded second derivative and $\lim_{t\rightarrow\infty}\lyap(t)$ exists and is finite then we have that $\lim_{t\rightarrow\infty}\dot{g}(t)=0$.
%\end{lemma}
%
%\begin{proof}
%Let's denote by $M\geq 1$  an upper bound on the second derivative of $g$.
%Suppose that the statement was not true. In this case, we would be able to find a sequence $\{t_n\}$ going to infinity such that $\dot{g}(t_n)$ remains bounded away from zero. Next, we can assume that $t_{n+1}>t_n+1$ and $\dot{g}(t_n)\geq \epsilon$
%for some $0 < \epsilon < 1$. If we define $g_{2n}=\lyap(t_n)$ and $g_{2n+1}=\lyap(t_n+\frac{\epsilon}{2M})$, then  a first application of the mean value theorem implies that $\dot{g}(t)\geq \frac{\epsilon}{2}$ for $t_n\leq t \leq t_n + \epsilon/2M$.
%\PM{Not sure I understand this, you mean this is the case \emph{for all} $t$?}
%A second application implies that $g_{2n+1}-g_{2n}\geq \frac{\epsilon^2}{4M}>0.$ Hence,  $\lim_{n\rightarrow\infty}g_n$ if it exists, is infinity. Therefore, the same holds for  $\lim_{t\rightarrow \infty}\lyap(t).$
%\begin{comment}
% does not exist either. Indeed, 
%%since $\lyap''$ is bounded by $M$ 
%we have that
%$\lyap'(t)\geq \frac{\epsilon}{2}$ for $t_n\leq t \leq t_n + \epsilon/2M$, which implies that $g_{2n+1}-g_{2n}\geq \frac{\epsilon^2}{4M}>0.$%\geq \epsilon^2/M >0$.
%\end{comment}  
%\end{proof}

We are now ready to prove that all interior initial conditions converge to the boundary.

\begin{theorem}
\label{thm:recurrence-boundary}
Let $\Phi$ denote the flow of the dynamic when applied to a zero-sum game.
%The probabilities of all strategies that do not appear in the support of any Nash equilibrium converge to zero as time goes to infinity.
If the game does not have a fully mixed Nash equilibrium, then
given any interior starting point $x\in \text{int}(\prod_{\play} \simplex(S_{\play}))$,
the orbit $\Phi(x,t)$ converges to the boundary of the state space.  
% game~\ref{eq:util} corresponds to a separable zero-sum game without a fully
%mixed Nash equilibrium, the system~\ref{eq:system} converges to the boundary of the state space.
Furthermore, if $q$ is an equilibrium of maximum support with $W_{\play}$ the respective supports of each agent's strategy 
then  $\omega(x)\subset \prod_{\play} \text{int}(\simplex(W_{\play}))$. 
\end{theorem}




\begin{proof}
Let $\eq=(\eq_{1},\eq_{2})$ be the \acl{NE} identified in \eqref{eq:dFench2} and let $\lyap(t) = \fench(y(t)) = \sum_{\play\in\players} \bracks{h_{\play}^{\ast}(y_{\play}(t)) - \braket{y_{\play}(t)}{\eq_{\play}}}$ denote the primal-dual coupling \eqref{eq:Fenchel} between $y(t)$ and $\eq$.
From \eqref{eq:dFench2}, we have that starting from any fully mixed strategy profile $x(0)\in \prod_{\play} \text{int}(\strats_{\play})$ and for all $t\geq 0$, $\lyap'(t) = \braket{\dot y}{\nabla\fench(y)}<0$.
%$\frac{d\big(D_{\mathrm{KL}}(q\|\Phi(x(0),t))\big)}{dt}<0$.
However, $\fench$ is bounded below by $-\sum_{\play} \max_{x_{\play}\in\strats_{\play}} h_{\play}(x_{\play})$, and since $\fench(y(t))$ is strictly decreasing, it must exhibit a finite limit.
%Since
%$\frac{d\fench}{dt}=  - \pay_{1}(\eq_{1},x_{2}) - \pay_{2}(x_{1},\eq_{2})$, and the time derivatives of $x_{\play}$  are bounded, $\fench(t)$
%has bounded second derivatives.
%Lemma \ref{eq:derivative} implies that $\lim_{t \rightarrow \infty} \frac{d\fench}{dt}= 0$.

\PM{What follows is new.}

We begin by noting that $x(t) = \choice(y(t))$ is Lipschitz continuous in $t$.
Indeed, $\payv$ is Lipschitz continuous on $\strats$ by linearity;
furthermore, since the regularizer functions $h_{\play}$ are assumed $\strong_{\play}$-strongly convex, it follows that $\choice_{\play}$ is $(1/\strong_{\play})$-continuous by standard convex analysis arguments \cite[Theorem~12.60]{RW98}.
In turn, this implies that the field of motion $\dynfield(y) \equiv \payv(\choice(y))$ of \eqref{eq:FRL} is Lipschitz continuous, so the dynamics are well-posed and $y(t)$ is differentiable.
Since $\dot y = \payv$ and, in addition, $\payv$ is bounded on $\strats$, we conclude that $\dot y$ is bounded so, in particular, $y(t)$ is Lipschitz continuous on $[0,\infty)$.
We thus conclude that $x(t) = \choice(y(t))$ is Lipschitz continuous as the composition of Lipschitz continuous functions.

We now further claim that $\lyap'(t)$ is also Lipschitz continuous in $t$.
Indeed, by \eqref{eq:dFench}, we have $\lyap'(t) = \sum_{\play\in\players} \braket{\payv_{\play}(x(t))}{x_{\play}(t) - \eq_{\play}}$;
since $\payv_{\play}$ is Lipschitz continuous in $x$ and $x(t)$ is Lipschitz continuous in $t$, our claim follows trivially.
Hence, by \cref{lem:derivative}, we conclude that $\lim_{t\to\infty} \lyap'(t) = \lim_{\to\infty} \sum_{\play\in\players} \braket{\payv_{\play}(x(t)}{x_{\play}(t) - \eq_{\play}} = 0$.
\PM{Rewrote the above.}
By \eqref{eq:dFench2} we know that for any point in the interior of the state space $\lyap'(t)=\frac{\partial L}{\partial t}<0$. Hence, this implies that  
 $y \in \omega(x(0))$ cannot lie in the interior of the state space (given that the embedded game does not have any interior Nash equilibrium). Moreover, we can repeat this argument for any subspace such that the restriction of the game on that subspace (when ignoring the strategies that are played with probability zero) does not have a fully mixed NE. 
Hence  the support of $y$ must be a subset of the support of $\eq$.
\GP{Expanded the above.}
The support of $\eq$ is not complete in 
the  first place since $\eq$ is not a fully mixed equilibrium, hence  $y$ must trivially lie on the boundary as well.
%Finally, since $D_{\mathrm{KL}}(q\|\Phi(x(0),t))$  %cannot grow past its initial value $D_{\mathrm{KL}}(q\|\Phi(x(0),0)$  %
%has a finite limit 
%each $y\in\omega(x(0))$ must assign positive probability to all strategies in the support of $q$.  
\end{proof}




==> Related.tex <==
%----------------------------------------------------------------------
%%% RELATED WORK
%----------------------------------------------------------------------
% !TEX root = ./Main.tex
%
%
Stuff here.
\PM{G, I increased the horizontal margins to the maximum allowable extent, but we really don't have enough space.
Maybe skip ``related work'' as a separate section and cram everything in the intro?
That said, I don't know what's the standard in SODA, so I'm leaving this up to you\dots}

==> Thanks.tex <==
%----------------------------------------------------------------------
%%% THANKS
%----------------------------------------------------------------------
% !TEX root = ./Main.tex
%
%
\thanks{P.~Mertikopoulos was partially supported by
the French National Research Agency (ANR) under grants
GAGA (ANR\textendash13\textendash JS01\textendash 0004\textendash 01)
and
ORACLESS (ANR\textendash 16\textendash CE33\textendash 0004\textendash 01).}
